Automatic Cell Counting in Flourescent Microscopy Using Deep Learning

Counting cells in fluorescent microscopy is a tedious, time-consuming task that researchers have to accomplish to assess the effects of different experimental conditions on biological structures of interest. Although such objects are generally easy to identify, the process of manually annotating cells is sometimes subject to arbitrariness due to the operator's interpretation of the borderline cases. We propose a Machine Learning approach that exploits a fully-convolutional network in a binary segmentation fashion to localize the objects of interest. Counts are then retrieved as the number of detected items. Specifically, we adopt a UNet-like architecture leveraging residual units and an extended bottleneck for enlarging the field-of-view. In addition, we make use of weighted maps that penalize the errors on cells boundaries increasingly with overcrowding. These changes provide more context and force the model to focus on relevant features during pixel-wise classification. As a result, the model performance is enhanced, especially in presence of clumping cells, artifacts and confounding biological structures. Posterior assessment of the results with domain experts confirms that the model detects cells of interest correctly. The model demonstrates a human-level ability inasmuch even erroneous predictions seem to fall within the limits of operator interpretation. This qualitative assessment is also corroborated by quantitative metrics as an ${F_1}$ score of 0.87. Despite some difficulties in interpretation, results are also satisfactory with respect to the counting task, as testified by mean and median absolute error of, respectively, 0.8 and 1.

==> 11_introduction.tex <==
\indent In the last years deep learning has developed into a powerful framework that is increasingly being used to analyse large scale-data. It has been successfully employed in scientific and commercial environments, with applications in image classification, and speech and handwriting recognition. In particular medical imaging and bioinformatics has been a fruitful field of research, with deep learning employed for the identification and segmentation of tumors \cite{brain_tumor} \cite{breast_cancer} \cite{ciresan2012deep} \cite{cirecsan2013mitosis} and generative models for image reconstruction \cite{reconstruction} and super-resolution \cite{super-resolution}.     \\
\indent One specific class of algorithm that has been used in conjunction with the research on medical imaging are convolutional neural networks (ConvNets or CNNs) \cite{jimenez} \cite{greenspan}. The literature of CNNs applied to medical image processing is quite extensive, as they have been particularly successful in detecting and classifying biological features \cite{lundervold} \cite{sainer} \cite{yadav}.  \\
\indent This work employs the use of this type of networks in order to identify and count cells into biological images, with  also providing a justification of the output number by means of a segmentation map that localizes the detected objects. This additional information is particularly relevant to support the results with a clear, visual evidence of which objects contribute to the final counts. \\
\indent The task of counting object in digital images is very common and useful for multiple applications, e.g. visual inspection of products, people and vehicle movements, classification of biological tissue, etc. Although recently machine learning approaches have rendered this task largely autonomous, there are still many fields which rely on humans to perform this job. This poses many problems, as this process may be very time-consuming depending on the number of available images. Moreover, the task becomes tedious when the objects to count appear in large quantities, thus leading to errors due to fatigue of the operators. On the other hand, sometimes there are images in which either the true objects are not clearly identifiable or background looks very similar to the structures of interest. When that is the case, the results become arguable and subjective due to the interpretation of such borderline cases. Therefore, the introduction of automatic procedures to detect and count objects in digital images would bring many benefits in such applications, speeding up the operations and lightening the efforts of researchers, as well as limiting fatigue errors and standardizing to the systematic effect of the model the arbitrariness due to multiple operators influence. \\
\indent The work presented in this paper focuses mainly on counting neuronal cells inside fluorescence microscopy images. Recently, Hitrec et al. \cite{hitrec2019neural} investigated the brain areas of mice that mediate the entrance into torpor and showed evidence of which networks of neurons are associated with this process.
Knowing and controlling the mechanisms that rule the onset of lethargy may have a significant impact when coming to applications to humans.
Being able to artificially induce hibernation may be crucial for a wide variety of medical applications, from intensive care to oncology, as well as space travels and more.
As a consequence,  their work arouses considerable interest on the topic and lays the foundations for novel and more in-depth studies. \\
\indent The counting of this type of cells however still heavily relies on the identification by a human operator. Each experiment requires the inspection hundreds of pictures of brain slices manually and annotate the cells of interest (stained cells) in each image. The procedure involves multiple steps to correctly acquire and process an image, in order to successfully count the number of neurons present in it (area selection, white balance, calibration, color correction, etc.) \cite{luppi1} \cite{luppi2} \cite{luppi3}. The drawback is that the method is time-consuming and prone to errors due to fatigue. Also, despite target structures are generally clearly identifiable and little practice is needed to train a new operator for the task, there is still a certain degree of intrinsic arbitrariness due to the operator's interpretation of borderline cases.\\
\indent For these reasons, our work aims at facilitating and speeding up future research in this and similar fields through the adoption of an intelligent system that counts the objects of interest without human intervention.  The advantages of doing so are two-fold. 
On one side, the benefit in terms of time and human effort saved through the automation of the task is evident.
On the other, using a Machine Learning (ML) model for different experiments would introduce a systematic ``operator" effect, thus limiting the arbitrariness of borderline cases both within and between experiments. \\
\indent There are three main supervised approaches that tackle the task of counting object in digital images. The first one, called \textit{counting-by-regression} has as input to the model the digital image with the number of present object inside it as label. The model is then trained to compute the raw count of objects directly. This method, however more easily implementable since it doesn't require ground truth maps doesn't provide any immediate justification of which elements are responsible for the final count. The second approach is called  \textit{counting-by-detection}, in which ground truth masks with bounding boxes that surround the object to detect are given as label to the model. The output of this model is an image in which pixels are classified into either signal (within the boxes) or background (outside) class. The raw count of objects is then extracted as the number of sets of connected pixel. This gives a direct explanation of which items are being counted.\\
\indent A further development on this approach is the so-called \textit{counting-by-segmentation}. Here, the labels consist in ground truth masks that include pixel-wise semantic representation of the objects. This produces a classification at a pixel level that makes it possible to distinguish also the exact boundaries of each object. The total number of objects is then retrieved again by looking at groups of connected pixels. \\
\indent There is a great significant of literature that testifies to the viability of these methods when it comes of detecting objects inside a digital picture. 
Lempitsky et al. \cite{lempitsky2010learning} were among the first to investigate automated approaches to count cells in digital images, and they showed how to get the total number of objects in an image starting from dot annotations. 
To this end, they introduced the concept of a density map as target. In particular, they adopted a simple linear regression model to reproduce a mixture of bidimensional Gaussians centered on dot annotations. The count was then retrieved by integrating over the predicted density map delivered by the model.
Another remarkable result was obtained by Seguí et al. \cite{segui2015learning}, who trained a convolutional neural network in a regression framework. Interestingly, the authors were able to show that the features learned during this process were also useful for object detection, meaning that the model actually learned what it was counting.
Arteta et al. \cite{arteta2016counting} successively discussed new approaches past the density map that focus on incorporating multiple dot annotations from noisy crowdsourced data, i.e. data annotated voluntarily by non-experts.
More recently, Cohen et al. \cite{paul2017count} presented a work in which they adopted a fully convolutional network derived from the Inception family %Szegedy et al.
\cite{szegedy2016rethinking}. In particular, they extended the idea of counting everything inside the receptive field as in \cite{segui2015learning}  by introducing redundant counts to make results more stable and reliable, thus transforming the concept of density map in \cite{lempitsky2010learning} into that of a count map. \\
\indent Moreover, some interesting approaches have been proposed over the years for the specific task considered in this paper, i.e. the detection of cells in fluorescent microscopy. A first approach was first described by Faustino et al. \cite{faustino} in 2009. They proposed a method that used the luminance information in the image to generate a graph representation that, after undergoing a mining process, was able to identify the cells inside the image. While this approach seemed to yield considerable results, it still required a great amount of mechanical feature engineering, therefore rendering it still not completely automated. In 2016 Kraus et al. \cite{kraus} suggested a method that combined deep CNNs with multiple instance learning
(MIL) in order to classify and segment microscopy images using only whole image level annotations. While this is certainly interesting as it requires only a handful of labelled images and not the segmentation or per-cell labels, this approach seems to be more directed to a multiclass cell detection of microscopy images. In 2017 Reza et al. \cite{reza} proposed a novel multiple-input multiple-output convolution neural network (MIMO-Net) that utilizes multiple resolutions of the input image, connects the intermediate layers for better localization and context and generates the output using multi-resolution deconvolution filters. As it required multiple resolution of the input image this method wasn't applicable to our case. In their 2019 paper, Riccio et al. \cite{riccio} proposed a new unsupervised method for the automatic cell segmentation and counting (CSC). While this would certainly bypass the need of ground truth masks, it still requires a certain amount of hand mechanical features engineering (division of the image into square patches, grey level clustering, adaptive thresholding, etc. ). \\
\indent The novel approach described in this paper is a development on the \textbf{counting-by-segmentation} approach. We implemented a modified version of Unet \cite{Unet} and Res-Unet \cite{res-unet} networks, which have already been proved as successful for the task of segmenting images of cells in biological tissues. Our framework leverages ground-truth maps as labels during training in order to produce also a justification of the counts in terms of localization of the detected objects. Moreover data augmentation as also been utilized in order to increase the efficiency the available annotated samples. as well as custom weight maps for the ground truth masks, in order to better segment clustered cells. We performed ablation studies and compared our technique with the aforementioned Unet-based networks  

